AMASS: Archive of Motion Capture as Surface Shapes

Large datasets are the cornerstone of recent advances in computer vision using deep learning. In contrast, existing human motion capture (mocap) datasets are small and the motions limited, hampering progress on learning models of human motion. While there are many different datasets available, they each use a different parameterization of the body, making it difficult to integrate them into a single meta dataset. To address this, we introduce AMASS, a large and varied database of human motion that unifies 15 different optical marker-based mocap datasets by representing them within a common framework and parameterization. We achieve this using a new method, MoSh++, that converts mocap data into realistic 3D human meshes represented by a rigged body model; here we use SMPL [doi:10.1145/2816795.2818013], which is widely used and provides a standard skeletal representation as well as a fully rigged surface mesh. The method works for arbitrary marker sets, while recovering soft-tissue dynamics and realistic hand motion. We evaluate MoSh++ and tune its hyperparameters using a new dataset of 4D body scans that are jointly recorded with marker-based mocap. The consistent representation of AMASS makes it readily useful for animation, visualization, and generating training data for deep learning. Our dataset is significantly richer than previous human motion collections, having more than 40 hours of motion data, spanning over 300 subjects, more than 11,000 motions, and will be publicly available to the research community.

==> sections/05_shape_estimation.tex <==
\subsection{Shape and Marker Estimation}
\label{sec:shape_estimation}
	Our method to estimate static shape is similar to MoSh~\cite{loper2014mosh} and for comparability we use a similar notation.
	We optimize poses $\Poses=\pose_{1\hdots F}$, and a single shape $\shape$ to fit the observed marker locations $\Obsmrks=\{\obsmrk_{i,t}\in \Obsmrks_t\}_{1\hdots F}$ for the $F=12$ randomly chosen frames, where $i$ indexes the markers in a frame; again we exclude soft-tissue deformations at this stage ($\dyna=0$).\\
	
	Following MoSh, we use a marker parametrization $\mrkmap(\latentmrk_i,\shape,\pose_t)$ that maps a latent, pose invariant representation of the markers, $\latentmrk_i$, to estimate their position in a posed frame, $\pose_t$, as simulated markers, $\simrk$. Subsequently, we utilize a single objective function to estimate 1) the time-independent parameters: body shape and latent-marker locations, and 2) time-dependent pose (including translation): 
    
        \begin{equation}
         \begin{split}
            E(\Latentmrks, \shape, \Poses_B, \Poses_H) 
            &= \datawt E_D(\Latentmrks, \shape, \Poses_B, \Poses_H) 
             + \shapewt E_{\shape}(\shape)  \\
            &+ {\posewt}_B E_{\pose_B}(\pose_B) 
             + {\posewt}_H E_{\pose_H}(\pose_H)     \\
            &+ \StoMwt E_{\StoM}(\Latentmrks, \shape)  
             + \initwt E_I(\Latentmrks, \shape)   .
            \label{eq:mosh_shape_obj}
         \end{split}
        \end{equation}
        Where $\Latentmrks=\{\latentmrk_i\}$ represents the set of all latent markers.
        The data term $E_D$ measures distance between \emph{simulated markers} $\mrkmap(\latentmrk_i,\shape,\pose_t)$ and observed markers $\obsmrk_{i,t}$
        \begin{equation}
            E_D(\Latentmrks, \shape, \Poses) = \sum_{i,t} \| \mrkmap(\latentmrk_i,\shape,\pose_t) - \obsmrk_{i,t}\|^2 .
        \label{eq:mosh_data_term}
        \end{equation}
    The remaining four are regularization terms as follows:
    \begin{itemize}
        \item $E_{\shape}$ is a Mahalanobis distance shape prior on the $\numBetas$ SMPL shape components.
        \item $E_{\pose_B}$ regularizes the body pose parameters (i.e. $69$ parameters, excluding translation and first $3$ pose parameters which define the model's world orientation). The prior term is the negative log-likelihood of a Gaussian Mixture Model with $8$ components learned from the CMU dataset. 
        \item $E_{\pose_H}$ regularizes hand pose parameters. 
        We project the full hand pose (i.e. $84$ hand parameters) into the low-D MANO pose space with $\numMANOOH$ dimensions per hand and compute the Mahalanobis distance in this space
                \begin{equation}
                    E_{\pose_H}(\pose_H) =
                     {\hat{\pose}_H}^T \Sigma_{\pose_H}^{-1} {\hat{\pose}_H},
                    \label{eq:mano_prior}
                \end{equation}
        where $\hat{\pose}$ represents the projection of the pose into the low-D space and $\Sigma_{\pose_H}$ is the diagonal covariance matrix of the low-D PCA coordinates (see ~\cite{MANO:SIGGRAPHASIA:2017}).
        \item $E_{\StoM}$ encourages latent markers to remain a prescribed distance $d$ from the body surface. We use an average value of $d=\mrkDistance$.
            \begin{equation}
                E_{\StoM}(\Latentmrks,\shape) 
                = \sum_{i} \| \mathrm{dist}(\latentmrk_i , S(\shape, \pose_0))-d\|^2
            \label{eq:mosh_s2m}
            \end{equation}
        where $\mathrm{dist}(\cdot)$ indicates point-to-surface distance. For every latent marker, we find the closest primitive (point, edge or plane) and analytically compute the distance partial derivatives w.r.t.~the model parameters. 
        \item $E_I$ penalizes deviations of latent markers from their initialized locations defined by the markerset.
    \end{itemize}

    In contrast to MoSh, the $\lambda$ hyper-parameters are determined using a training set of 4D scans that are captured with synchronized mocap. The $\lambda$ values are optimized to reduce reconstruction error of shapes estimated with the above method when compared against ground truth validation scans. Details about the synchronized 4D scan dataset (SSM) and hyper-parameter search are given in Sec.~\ref{subsec:SSMdata} and Sec.~\ref{subsec:gridsearch} respectively. 
    Note that a standard $46$-markerset was used to determine the $\lambda$ weights during the hyper-parameter search. 
    The data term, $E_D$, in  Eq.~\ref{eq:mosh_data_term} uses a sum of squared distances, which is affected by the number of markers in the observed mocap sequence. 
    To deal with varying numbers of markers, we automatically vary the weight of this term by scaling this term by a factor $b = 46/n$, where $n$ is the number of observed mocap markers.
    
    To help avoid local optima, we minimize Eq.~\ref{eq:mosh_shape_obj} using $4$ stages of graduated optimization. Using the Threshold Acceptance method \cite{dueck1990threshold} as a fast annealing strategy, we start with strong regularization and weaker data term weights, gradually decreasing the regularization and making the data weight stronger at each stage. We increase $\datawt$ by multiplying it by a constant factor $s=2$ while dividing the regularizes by the same factor at each of the $4$ stages of annealing. 
    The weights at the final iteration are as follows:

\begin{multline}
        \datawt=600 \times b, 
        \shapewt=1.25, 
        {\posewt}_B=0.375, 
        {\posewt}_H=0.125,\\ 
        \initwt=37.5, 
        \StoMwt=1e4 
\end{multline}

The surface distance regularization weight, $\StoMwt$, remains constant throughout the optimization. 
Note that the number of hand pose components are set to $0$ for the first two stages of the graduated optimization to allow the remaining parameters (body pose, body shape and estimated marker positions) to reach a closer fit to the observed data. The $\numMANOOH$ hand pose components are then added into the optimization during the final two iterations.





==> sections/06_pose_estimation.tex <==
\subsection{Model Fitting}
\label{sec:pose_estimation}

    Once the static shape of a subject and refined marker locations $\latentmrk_i$ on the body have been computed, we estimate the pose of the body across each of the mocap sequences. In this stage, the marker locations and shape parameters of the model are assumed constant over time so they are held fixed. 
    The objective at this stage optimizes pose for each frame of mocap in the sequence as opposed to the $12$ frames optimized simultaneously during shape stage.

    Using a similar objective as defined for the shape estimation stage in Eq.~\ref{eq:mosh_shape_obj}, we remove the marker and shape optimization terms, $E_I$, $E_{\StoM}$ and $E_{\shape}$, leaving behind the data term and pose prior, $E_D$, $E_{\pose}$. 
    In contrast to MoSh, here we now also optimize for the soft-tissue deformation coefficients, $\dyna$. We add a prior and a temporal smoothness terms, $E_{\dynaConst}(\dyna)$ and $E_{\dynaConst}$ respectively, to regularize the soft-tissue deformations.
	Like MoSh, we add a temporal smoothness term for pose as well, $E_{\poseConst}$, to help reduce the effect of jitter noise in the mocap marker data. 
The objective function is then
        \begin{equation}
         \begin{split}
            E(\pose_B, \pose_H, \dyna) 
            &= \datawt E_D(\pose_B, \pose_H, \dyna) \\
            &+ {\posewt}_B E_{\pose_B}(\pose_B) 
             + {\posewt}_H E_{\pose_H}(\pose_H) \\
            &+ \poseConstwt E_{\poseConst}(\pose_B, \pose_H) \\ 
            &+ \dynawt E_{\dyna}(\dyna) + \dynaConstwt E_{\dynaConst}(\dyna) 
            \label{eq:mosh_pose_obj}
         \end{split}
        \end{equation}
where the data term $E_D$ is defined in Eq.~\ref{eq:mosh_data_term}.

The body and hands pose prior terms, $E_{\pose_B}$ and $E_{\pose_H}$, for this stage are the same as described in the shape estimation stage, Sec.~\ref{sec:shape_estimation}. 
To regularize the soft-tissue coefficients, we add a Mahalonobis distance prior on the $8$ DMPL coefficients.
        \begin{equation}
            E_{\dyna}(\dyna) =
            \dyna_t^T \Sigma_{\dyna}^{-1} \dyna_t,
            \label{eq:dyna_prior}
        \end{equation}
where the covariance $\Sigma_{\dyna}$ is the diagonal covariance matrix from the DYNA dataset~\cite{Dyna:SIGGRAPH:2015}. 


The initialization and fitting for the first frame of motion undergoes a couple of extra steps compared to the rest of the motion. 
For the first frame, we initialize the model by performing a rigid transformation between the estimated and observed markers to repose the model from its rest pose $\mathbf{T}$ to roughly fit the observed pose. Then we use a graduated optimization for the objective defined above with only the data and body pose prior terms, while ${\posewt}_B$ is varied from $[10, 5, 1]$ times the final weight.
For each of the subsequent frames, we initialize with the solution of the previous frame to estimate the pose and soft-tissue parameters.

The per-frame estimates of shape and pose after the first frame are carried out in two steps. During the first step, we set the dynamics weights, $\dynawt=0$ and $\dynaConstwt=0$, allowing us to optimize only pose. This prevents the dynamics components from trying to explain translation or large pose changes between consecutive frames. Then, we add the dynamics, $\dyna$, and the dynamics smoothness terms into the optimization for the final optimization of pose and shape.

 The optimal $\lambda$ weights for data term $\datawt$, pose prior $\posewt$ and soft-tissue dynamics prior $\dynawt$ were set using the SSM training set to reduce reconstruction error of estimated posed meshes from MoSh++ against ground truth 3D scans as explained in Sec.~\ref{subsec:gridsearch}. 
    The velocity constancy weights $\poseConstwt$ and $\dynaConstwt$ depend on the mocap system calibration and optical tracking quality, data frame rate, and the types of 
    
    
    
    . Therefore, these values could not be optimized using just one source of data, so we empirically determined them through experiments on different datasets of varying frame rates and motions. 

    The final weights determined for the MoSh++ pose estimation stage are:
    
	\begin{multline}
        \datawt=400 \times b , 
        {\posewt}_B=1.6 \times \posecpl, 
        {\posewt}_H=1.0 \times \posecpl, 
        \poseConstwt=2.5,  \\
        \dynawt=1.0, 
        \dynaConstwt=6.0 .
	\end{multline}


Similar to $b$, which adjusts the weight of the data term to varying markersets, $q$ is a weight-balancing factor for the pose prior $\posewt$. 
During a mocap session, markers may get occluded by the body due to pose. If multiple markers of a particular body part are occluded simultaneously, the optimization may result in unreliable and implausible poses, such as the estimated pose shown in Fig.~\ref{fig:pose_vary_factor} (left). 
    To address this, we introduce a coefficient $\posecpl=1 + \big(\frac{x}{|\Obsmrks|} * 2.5 \big)$, where $x$ is the number of missing markers in a given frame, $|\Obsmrks|$ are the number of total observed markers. This updates the pose prior weight as a factor of the number of missing markers. 
The more markers that are missing, the higher this weights the pose prior.
    This term can increase the prior weight by up to a factor of $\posecpl=3.5$, in the worse case scenario where $x=|\Obsmrks|$, and goes down to having no effect, $\posecpl=1.0$ when all session markers are visible $x=0$. An example of the pose-estimation with this factor is shown in Fig.~\ref{fig:pose_vary_factor} (right). 
    
    \begin{figure}[t]
    \centerline{
        \includegraphics[height=1.8in]{images/pose_stage/pose_vary_factor.png} }
    \caption{ Pose estimation with heavy marker occlusion. Pose optimization with constant pose prior weight $\posewt$ (left), variable pose prior weight $\posewt$ (right). $\posewt$ is allowed to vary as a factor of fraction of visible markers resulting in more plausible poses even when toe markers (right foot) and all foot markers (left foot) are missing. Estimated and observed markers are shown in red and green, respectively.}
   
    \label{fig:pose_vary_factor}
    \end{figure}


    \label{sec:DMPL}







When hand markers are present, MoSh++ optimizes the hand pose parameters in the same way as all the other pose parameters except that we use $\numMANOOH$ dimensions of MANO's \cite{MANO:SIGGRAPHASIA:2017} low-dimensional representation of the pose.
This is added to Eq.~\ref{eq:dyna_prior} when hand markers are present.
For this extended pose space, we found that the data term and pose prior weights had to be modified, with $\datawt=150$ and $\posewt=1.5$. Since these could not be determined using the SSM dataset (SSM does not contain hand mocap markers), the values had to be defined empirically. The remaining terms remain the same.

In cases where there are no markers present on the hands of the recorded subjects,  the hand pose is set to the average (relaxed) pose of the MANO model.





    
    


    

==> sections/glossary.tex <==
 
 
\newglossaryentry{latex}
{
    name=latex,
    description={Is a mark up language specially suited 
    for scientific documents}
}
 
\newglossaryentry{maths}
{
    name=mathematics,
    description={Mathematics is what mathematicians do}
}
 
 


==> sections/marker2model.tex <==
\subsection{Accuracy of Marker-to-Model Correspondences}


We evaluate the accuracy of automatically generated marker-to-model correspondences in terms of classification accuracy as well as mesh reconstruction error compared to manually placed correspondences.
For classification, we report two types of accuracy measures. 
1) Marker correspondence accuracy: shows how accurately our correspondence solver fits to the manual labels for all the markers in the entire mocap dataset, 
2) Motion sequence accuracy: measure how many motions we can consider accurately labelled in a given dataset. For this evaluation, we consider a motion a failure if more than $10\%$ of the auto-correspondence labels do not match up with the mannually assigned labels of the original dataset. For instance if more than $4$ markers in any CMU motion sequence (of total $41$ markers) do not match, we report it as a failure in this evaluation.
To do these evaluations, we replace the labels in the marker superset with marker labels of the mocap dataset that we are comparing to, and report how accurately the correspondence solver solution matched the manual labels. We report these errors for $5$ different datasets in the $\database$ database: SSM, BML, CMU, MPI-HDM05 and MPI-MoSh.
\begin{itemize}
    \item SSM ($30$ motions)
        marker accuracy: $90.45\%$,
        motion sequence accuracy: $95.03\%$
    \item BML ($3387$ motions)
        marker accuracy: $95.17\%$, 
        motion sequence accuracy: $97.99\%$
    \item CMU ($2133$ motions)
        marker accuracy: $89.02\%$,
        motion sequence accuracy: $86.83\%$
    \item MPI-HDM05 ($294$ motions)
        marker accuracy: $100\%$,
        motion sequence accuracy: $100\%$
    \item MPI-MoSh ($78$ motions)
        marker accuracy: $95.01\%$, 
        motion sequence accuracy: $92.31\%$
    \item TCD ($62$ motions)
        marker accuracy: $93.15\%$,
        motion sequence accuracy: $82.25\%$
\end{itemize}

The error in classification can be conflated due to signal noise in the mocap system, errors in the orginal manual labelling of these datasets, and additional virtual markers that added to some of the archival datasets, meaning that the ceiling may not be $100\%$. 
We observe that misclassification errors occur for nearby markers, mostly on the wrist. Or in some cases, the misclassification is not actually an error, but a variation of marker placement / marker labeling between the superset markers and manual labels. 
But, even for mislabeled markers, we find that this initialization is sufficiently good since during the MoSh++ shape estimation stage, we allow the markers to travel along the surface to improve marker location estimation. 
There are however failures in cases when there may be an equal chance of the body getting fit to the wrong orientation (front to back), Fig.\ref{fig:lm_failure}. 
\textcolor{red}{We do not exclude these from the dataset. we could discard moshed files the fitting error goes too far beyond a thrershold}

We also evaluate the success of the automatic correspondences by evaluating the mesh reconstruction error
. In the end, this is what matters most.
We manually labeled a single motion for each subject in the SSM dataset, and estimated shape from this motion alone for a comparison of reconstruction error between manually and automatically labeled mocap. 
We report the errors 1) using our automatic correspondence solver and 2) manually assigned correspondences. We pick the same frames during shape reconstruction for testing both the methods.
Automatic correspondences produce a reconstruction error of $7.6mm$. 
This is slightly better than the reconstruction error using manually assigned labels, $8.1mm$.
The automatic correspondences finds a better matches for the observed markers in the marker superset than the manually assigned labels, especially because the manual placement of the markers during the mocap sessions varies per session. This means that the correspondences computed using the MoSh++ auto-correspondence method can generate better reconstruction results.

\begin{figure}
    \includegraphics[width=3.4in]{images/autolabeling/lm_failure.png}
    \caption{{\bf Auto-correspondence Failures:}
    {\em Two correct fitted poses (left) and two wrong fitted poses (right) are shown. Each marker is colored the same color in each frame to illustrate the marker trajectory. %
    Failures in fitting occur in cases when front and back orientation of the subject is hard to detect.}
    }
    \label{fig:lm_failure}
\end{figure}

